Coupled Control Systems: Periodic Orbit Generation with Application to Quadrupedal Locomotion

A robotic system can be viewed as a collection of lower-dimensional systems that are coupled via reaction forces (Lagrange multipliers) enforcing holonomic constraints. Inspired by this viewpoint, this paper presents a novel formulation for nonlinear control systems that are subject to coupling constraints via virtual "coupling" inputs that abstractly play the role of Lagrange multipliers. The main contribution of this paper is a process---mirroring solving for Lagrange multipliers in robotic systems---wherein we isolate subsystems free of coupling constraints that provably encode the full-order dynamics of the coupled control system from which it was derived. This dimension reduction is leveraged in the formulation of a nonlinear optimization problem for the isolated subsystem that yields periodic orbits for the full-order coupled system. We consider the application of these ideas to robotic systems, which can be decomposed into subsystems. Specifically, we view a quadruped as a coupled control system consisting of two bipedal robots, wherein applying the framework developed allows for gaits (periodic orbits) to be generated for the individual biped yielding a gait for the full-order quadruped. This is demonstrated through walking experiments of a quadrupedal robot in simulation and on rough terrains.

==> sections/0Intro.tex <==
\section{Introduction} 
\label{sec:intro}


To achieve dynamic walking on high-dimensional robotic systems, hybrid zero dynamics (HZD) has proven to be a successful methodology as a result of its ability to make theoretic guarantees \cite{Westervelt2007a, Grizzle2014Models, ames14CLF} and yield walking for complex humanoids \cite{Sreenath2011, reher2016realizing}. 
% \cite{Sreenath2011, %ma2017bipedal, reher2016realizing}. 
The main idea behind this approach is that the full-order dynamics of the robot can be reduced to a lower-dimensional surface on which the system evolves. The system can then be studied via the low-dimensional dynamic representation and, importantly, guarantees made can be translated back to the full-order dynamics, i.e., periodic orbits (or walking gaits) in the low-dimensional system imply corresponding periodic orbits in the full-order system. The goal of this paper is to capture this dimension reduction in a more general context---that of \systems, which capture the ability to decompose a complex system into low-dimensional subsystems. 


Another means of dimension reduction for robotic systems comes from isolating subsystems and coupling these subsystems at the level of reaction forces, i.e., Lagrange multipliers that enforce holonomic constraints. This is the idea underlying the highly efficient method for calculating the dynamics of robotic systems: Spatial vector algebra \cite{featherstone2014rigid}. For example, a double pendulum can be decomposed into two single pendula connected via a constraint at the pivot joint \cite{ganesh2007composition}. More generally, one can consider two equivalent ways of expressing the dynamics of a robotic system \cite{Murray1994mathematical}: 
\par\vspace{-4.3mm}{\small\begin{align*}
    \underbrace{D(q) \ddot{q} + H(q,\dot{q}) = u}_{\textrm{Full-Order Dynamics}} 
    \Leftrightarrow 
    \underbrace{\begin{dcases}
    D_i(q_i) \ddot{q}_i + H_i(q_i,\dot{q}_i) = u_i + J_{h_i}^\top \lambda  \\
    \qquad \qquad  \mathrm{s.t.} \qquad  h(q)= 0
    \end{dcases}}_{\textrm{Reduced-Order Coupled Dynamics}}
\end{align*}}%
\vspace{-3.4mm}\par\noindent
for $i = 1,2$, where $h$ is a coupling (holonomic) constraint that is enforced via the Lagrange multiplier $\lambda$ allowing for the higher-dimensional $q$ to be decomposed into lower-dimensional $q_i$, i.e., $q = (q_1,q_2)$. For example, a quadrupedal robot can be decomposed into two bipeds as in \figref{fig:frontPage}. Thus, if one can make guarantees on the reduced-order coupled systems, they can be translated to the full-order dynamics. 
% This idea has also, again, proven successful in robotic walking when dealing with what are referred to as the ``pinned'' and ``unpinned'' models---this success has been especially prevalent in the context of constructing efficient nonlinear constrained optimization problems, especially for bipedal walking robots that utilize hybrid zero dynamics \cite{hereid_dynamic_TRO}.



The study of coupled dynamic and control systems has a long and rich history from which the framework presented in this paper has taken inspiration. The most prevalent example is that of multi-robot systems \cite{mesbahi2010graph}, and specifically the consensus problem \cite{ren2005survey}. 
%\cite{olfati2004consensus,ren2005survey}, along with nonlinear extensions \cite{yu2011consensus}. 
Interconnected systems have also been well-studied \cite{antonelli2013interconnected}. 
%, including extensions over graphs \cite{langbort2004distributed}.  
% Examples of this include nonlinear oscillators \cite{fujisaka1983stability}, with Kuramoto oscillators of particular note \cite{chopra2009exponential}, wherein synchronization can be viewed as a coupling constraint as considered here. 
In the context of mechanical and robotic systems on graphs, network synchronization has been considered \cite{chung2009cooperative}.
% and along with the synchronization of Lagrangian systems using passivity \cite{spong2007synchronization}.  
Port-Hamiltonian systems also capture the notion of coupling present in general mechanical systems \cite{van2014port}. 
Finally, in related work, the coordination of quadruped and human reaction forces has recently been studied \cite{hamed2019hierarchical}. 
While not explicitly discussed due to space constraints, many of these formulations fit within the general setting of coupled control systems presented here. 


\begin{figure}[t!]
	\centering
	\includegraphics[width=0.43\textwidth]{Figures/Intro_quad_small_grey_compressed.png}
	\vspace{-2.5mm}
	\caption{Conceptual illustration of the full body dynamics decomposition, where the 3D quadruped --- the Vision 60 --- is decomposed into two constrained 3D bipedal robots.}
	\label{fig:frontPage}
	\vspace{-4.8mm}
\end{figure}

\begin{comment}
This paper generalizes the aforementioned methods --- zero dynamics and system decomposition through coupling constraints --- and unifies them through a novel formulation: {\it coupled control systems}. 
% Specifically, we consider the full-order dynamics represented by a (bidirected) graph on which there is a nonlinear control system on every vertex including internal and coupling dynamics and constraints on every edge. 
We then utilize zero dynamics to reduce to a subsystem dependent on coupling constraint which is then eliminated via coupling relations to yield the final isolated subsystem. %, i.e., a subsystem that no longer depends on the coupling constraint and is of lower dimension than the original full-order coupled dynamics from which it was derived. 
The main result of this paper is that trajectories of the isolated subsystem are trajectories of the full-order system, and thus periodic orbits on the subsystem yield periodic orbits on the full-order system. This result is leveraged to construct a nonlinear optimization problem utilizing collocation methods to generate these periodic solutions. 
\end{comment}


This paper generalizes the aforementioned methods --- zero dynamics and system decomposition through coupling constraints --- and unifies them through a novel formulation: {\it coupled control systems}. We then utilize zero dynamics to reduce to a subsystem dependent on coupling constraint which is then eliminated via coupling relations to yield the final 
isolated subsystem. The main result of this paper is that solutions of the isolated subsystem are solutions of the full-order system, and thus periodic orbits on the subsystem yield periodic orbits on the full-order system. This result is leveraged to construct a nonlinear optimization problem utilizing collocation methods to generate these periodic solutions. 



Our motivating application is gait (periodic orbit) generation for quadrupedal robots.
% Having established the formal underpinnings of \system along with their algorithmic instantiation, we return to the application that motivated the framework formulated in this paper: gait (periodic orbit) generation for quadrupedal robots. 
%
Previously, HZD methods were applied to quadrupedal walking \cite{ma2019First}; yet the high dimensionality of this system made it computationally expensive to generate gaits when compared to their bipedal analogs. To address this shortcoming, recent work has aimed at decomposing quadruped into bipedal robots \cite{ma2019bipedal}---it is this methodology that this paper formalizes and extends. 
% 
Therefore, we consider a quadrupedal robot utilizing the \system~ paradigm, wherein this system can be reduced to lower-dimensional subsystems on which periodic orbits (gaits) can be generated. % that are thus walking gaits for the full-order quadruped dynamics. 
We demonstrate the results through the realization of these generated gaits experimentally to achieve stable walking on rough terrains. 



% \red{The paper is structured as follows. Along the process, we illustrate the theoretical concepts with an application to periodic orbit generation for quadrupedal robots. 
% Sec.\ref{sec:def} introduces the fundamental concepts of \systems, and the means in which to reduce them to isolated systems. 
% % are presented in Sec.\ref{sec:isolating}. 
% This section also presents the main result of the paper: that solutions to the isolated subsystem (e.g., periodic orbits) are solutions to the original full-order coupled control system. This leads to the formulation of an optimization problem in Sec.\ref{sec:opt} for generated periodic orbits via the isolated subsystems. 
% % A specific instance---symmetric coupled control systems---are considered too. 
% This lays the groundwork for the application of the ideas in this paper to quadrupedal robots in Sec.\ref{sec:quad}. In this section, the methods developed are used to generate walking gaits which are demonstrated experimentally. % We finish with conclusions in Sec.\ref{sec:conclusion}. 



\begin{comment}
Notes: references here so they can be worked into intro later. 
\begin{itemize}
    \item Kuramoto Oscillators (work of Spong, etc.).  \cite{chopra2009exponential} and coupled oscilators \cite{fujisaka1983stability}
    \item Networked control systems, i.e., multi-robot systems (Egerstedt, etc.) \cite{mesbahi2010graph}, consensus \cite{olfati2004consensus} and consensus for nonlinear dynamics \cite{yu2011consensus,yu2009second} (fits within the formulation of this paper). 
    
    \item Switched and multiple Lyapunov functions \cite{long2017multiple}. 
    \item Port-hamiltonian systems \cite{van2014port}
    \item Network synchronization for robotic systems \cite{chung2009cooperative} and Lagrangian systems using passivity \cite{spong2007synchronization}
    %\item Hybrid zero dynamics  and Lyapunov stability and stabilization with control Lyapunov functions \cite{ames14CLF}
    %\item decoupling robotic systems via Lagrangian multipliers that enforce holonomic constraints \cite{Murray1994mathematical} and Spatial vector algebra \cite{featherstone2014rigid}
    \item Recent results on quadrupeds viewed as coupled bipeds with experimental realization \cite{ma2019bipedal} rather then applying HZD to the full-order dynamics \cite{ma2019First}
\end{itemize}
\end{comment}


==> sections/4quad.tex <==
% \section{Application to Quadrupeds} \label{sec:quad}


% To illustrate the methodology presented in this paper, specifically (symmetric) coupled control systems, we will present an approach that decomposes symmetric rigid body systems, i.e., robotic systems, into subsystems for the purposes of periodic orbit generation. In particular, we are interested the application to quadrupedal robots, viewed as coupled control systems, with each isolated subsystem consisting of a bipedal robot. We will generate periodic motions this subsystems which will yield walking gaits on the original quadrupedal robot as will be demonstrated experimentally. 
% in robotic locomotion that are often modeled as hybrid dynamics, which is an alternating sequence of continuous and discrete time dynamics. 
% In this section we apply the proposed method to design stabilizing controllers for a quadrupedal robot (see \figref{fig:quad}).

% To illustrate the methodology presented in this paper, we show an approach that decomposes robotic systems, into subsystems for the purposes of periodic orbit generation. In particular, we are interested the application to quadrupedal dynamics, finding the solutions to which are computationally expensive due to its high degrees of freedom \cite{ma2019First}. In this section, we view a quadruped as a CCS, with each isolated subsystem being a biped. We then generate periodic motions for this subsystem which will yield walking gaits on the original quadruped, as will be demonstrated experimentally. 


\begin{example} 
% \newsec{Gait Generation. } 
We now utilize the optimization method in Sec.\ref{sec:opt} to find a periodic solution to the quadrupedal dynamics, representing the ambling motion. This is by leveraging the \eqref{eq:generalOPT} with some additional constraints specific to walking. That is, dynamics of quadrupedal locomotion including both continuous and discrete dynamics, forming a \textit{hybrid control system}. 
%
Concretely, we leverage the subsystems representing the front and rear bipeds: $\bipedz{\rmf}$ and $\bipedz{\rmr}$, as given in \eqref{eq:bizieom}. Note that these subsystems are still coupled through $\lambda$---while this could be explicitly solved for via \eqref{eq:lambdaForce}, we keep it implicit due to the complexity of inverting the mass-inertia matrix for this particular robotic application. %
The \ith subsystem yield (C.1), (C.2) and (C.3) for \eqref{eq:generalOPT}. Specifically, we have the decision variables for all of the grid indices  $\id=0,1,...5$: 
\par\vspace{-4mm}{\small 
\begin{align*}
    \vi = \{q_\rmf^\id, \dot{q}_\rmf^\id, \xi_\rmr^\id, \dot\xi_\rmr^\id, u_\rmf^\id, F_\rmf^\id, F_\rmr^\id, \alpha_\rmf, \lambda_e^\id \},
    ~\mathbf{X}=\{\vi\}_{\id=0,\ldots5}. 
\end{align*}}% 
% 
When posing the \eqref{eq:generalOPT}, we pick cost function as the acceleration of the torso orientation to yield a less energetic motion for the ease of experiments. 
As a result, the optimization problem converged to a solution to the original quadrupedal dynamics, that is a periodic orbit (shown in \figref{fig:walk2exp}). 
% The computation test was conducted on a Linux laptop with an i7-6820HQ CPU @$2.70$ GHz and $16$ GB RAM. 
We report that the computation takes 17.6seconds and 295 iterations of searching. Comparing to the traditional full-model based optimization methods \cite{ma2019First}, whose fastest performance was 42 seconds, the coupled system optimization is over $50\%$ faster.  




% \newsec{Trajectory optimization. } We now pose the \eqref{eq:generalOPT} as:
% \par\vspace{-4mm}{\small 
% \begin{align}  \label{eq:quadOPT}
%     \underset{\mathbf{X}}{\operatorname{argmin}}\ \ & A_{\mathrm{base}}( \mathbf{X} ) & \\
%     \text{s.t.\ \ }
%     & \text{(C.1),(C.2),(C.3),(C.4)}              & \notag\\
%     % & F_{\text{zero}}(\vartheta^\id) = 0         &\id = 0,1,\ldots,\rmK \tag{C.1}\\
%     % & F_{\text{dyn}}(\vi)= 0                     &\id = 0,2,4,\ldots \tag{C.2}\\
%     % & d(\mathbf{X}) = 0                          & \tag{C.3} \\
%     %& \vartheta^\id \in \X\times\Z\times\Us       &\id=0,1,\ldots,5 \tag{C.4}\\
%     & p(q_i^\id) \geq 0                           &\id=0,1,\ldots,5 \tag{C.5}\\
%     & b(q_i^0, \dot{q}_i^0, q_i^5, \dot{q}_i^5)=0 &                 \tag{C.6}
% \end{align}}%
% where the cost function $A_{\mathrm{base}}(\cdot)\in\R$ represents the acceleration of the torso orientation to yield a less energetic motion for the ease of experiments; 
% (C.4) defines the feasible configuration space and available motor torques for the physical robot;  
% (C.5) defines the ground clearance of the swing foot to be higher than 10cm and the friction cone condition. 
%
% Note that we picked $\rmK=5$. 
% \textit{Note that, we did not optimize the controller $\uZ_j$ for invariance}

% As a result, \eqref{eq:quadOPT} converged to a solution to the original quadrupedal dynamics, that is a periodic orbit (shown in \figref{fig:walk2exp}). 
% % The computation test was conducted on a Linux laptop with an i7-6820HQ CPU @$2.70$ GHz and $16$ GB RAM. 
% We report that the computation takes 17.6 seconds and 295 iterations of searching. Comparing to the traditional full-model based optimization methods \cite{ma2019First}, whose fastest computation was 42 seconds, the coupled system optimization is over $50\%$ faster.  



\end{example}
